Symmetric Replay Training: Enhancing Sample Efficiency in Deep Reinforcement Learning for Combinatorial Optimization

Deep reinforcement learning (DRL) has significantly advanced the field of combinatorial optimization (CO). However, its practicality is hindered by the necessity for a large number of reward evaluations, especially in scenarios involving computationally intensive function assessments. To enhance the sample efficiency, we propose a simple but effective method, called symmetric replay training (SRT), which can be easily integrated into various DRL methods. Our method leverages high-reward samples to encourage exploration of the under-explored symmetric regions without additional online interactions - free. Through replay training, the policy is trained to maximize the likelihood of the symmetric trajectories of discovered high-rewarded samples. Experimental results demonstrate the consistent improvement of our method in sample efficiency across diverse DRL methods applied to real-world tasks, such as molecular optimization and hardware design.

==> packages.tex <==

\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{subcaption}

\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{multirow}
\usepackage{makecell}

\usepackage{enumitem}

% \PassOptionsToPackage{numbers, compress}{natbib}
\usepackage{xcolor} 
\usepackage[capitalise]{cleveref}

\usepackage{amsthm}
\theoremstyle{definition}
\newtheorem{definition}{Definition}%[section]
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}{Proposition}[section]

\usepackage{algorithm}
\usepackage{algpseudocode}

\usepackage{float}
\newfloat{algorithm}{t}{lop}

\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}

\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}
% \algnewcommand{\LineComment}[1]{\State $\backslash* \qquad$ \textsc{#1} $\qquad *\backslash$}
\algnewcommand{\LineComment}[1]{\STATE \textcolor{purple}{\(\triangleright\) \quad \textsc{#1}}}

\usepackage{wrapfig}
% \usepackage{floatrow}
% Table float box with bottom caption, box width adjusted to content
% \newfloatcommand{capbtabbox}{table}[\captop][\FBwidth]

==> tables/diff_trans.tex <==
% \begin{tabular}{lcccc}
% \toprule
%  & \multicolumn{2}{c}{Avg. Cost ($\downarrow$)} & \multicolumn{2}{c}{Difference ($\downarrow$)}   \\
% \cline{2-3} \cline{4-5}
%  & 100K & 2M  & 100K & 2M \\
% \midrule
% MaxEnt & 6.591 $\pm$ 0.055 & 6.032 $\pm$ 0.008 & 21.608 $\pm$ 2.455 & 15.349 $\pm$ 0.328 \\
% Sampling & 6.595 $\pm$ 0.116 & 6.024 $\pm$ 0.009 & 19.535 $\pm$ 1.489 & 15.327 $\pm$ 0.406 \\
% Adversarial & \textbf{6.516 $\pm$ 0.044} & \textbf{6.018 $\pm$ 0.007} & \textbf{10.716 $\pm$ 0.382} & \textbf{8.368 $\pm$ 0.439} \\
% \bottomrule
% \end{tabular} 

\begin{tabular}{lcc}
\toprule
%  & \multicolumn{2}{c}{Avg. Cost ($\downarrow$)} & \multicolumn{2}{c}{Difference ($\downarrow$)}   \\
% \cline{2-3} \cline{4-5}
 & 100K & 2M \\
\midrule
MaxEnt & 21.608 $\pm$ 2.455 & 15.349 $\pm$ 0.328 \\
Sampling & 19.535 $\pm$ 1.489 & 15.327 $\pm$ 0.406 \\
Adversarial &  \textbf{10.716 $\pm$ 0.382} & \textbf{8.368 $\pm$ 0.439} \\
\bottomrule
\end{tabular} 



==> tables/dist_euclidean.tex <==

% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{llccccc}
% \toprule[1.0pt]
%  &  &  & \multicolumn{2}{c}{$N=50$} &  \multicolumn{2}{c}{$N=100$}\\
% \cmidrule(lr{0.2em}){4-5}\cmidrule(lr{0.2em}){6-7}

% Task & Method & Trained Size & Avg. Cost & L1 Dist.  & Avg. Cost & L1 Dist. \\
% \midrule[0.8pt]
% \multirow{4}{*}{TSP} & AM Critic & 50 & 6.1153 & 144.4978 & 8.8801 & 315.5329 \\
% & \ours{} (ours) & 50 & \textbf{6.0458} & \textbf{30.4985} & \textbf{8.726} & \textbf{49.8098} \\
% \cmidrule(lr{0.2em}){2-7}
% & AM Critic & 100 & 6.6262 & 275.9329 & 9.1065 & 569.7021 \\
% & \ours{} (ours) & 100 & \textbf{6.1988} & \textbf{32.5435} & \textbf{8.6004} & \textbf{42.7087} \\
% \midrule[0.8pt]
% \multirow{4}{*}{CVRP} & Sym-NCO & 50 & 11.8829 & 753.2776 & 18.5932 & 1507.4207 \\
% & \ours{} (ours) & 50 & \textbf{11.7830} & \textbf{558.8633} & \textbf{18.4096} & \textbf{1079.0616} \\
% \cmidrule(lr{0.2em}){2-7}
% & Sym-NCO & 100 & 12.4599 & 687.2557 & 18.6265 & 1415.3947 \\
% & \ours{} (ours) & 100 & \textbf{12.2693} & \textbf{549.0758} & \textbf{18.4799} & \textbf{1101.5375} \\
% \bottomrule[1.0pt]
% \end{tabular}\label{tab:sym-measure}
% }



\resizebox{0.75\linewidth}{!}{
\begin{tabular}[t]{lcccccc}
\toprule[1.0pt]
 &  & \multicolumn{2}{c}{$N=50$} &  \multicolumn{2}{c}{$N=100$}\\
\cmidrule(lr{0.2em}){2-4}\cmidrule(lr{0.2em}){5-7}
Method & Trained Size & Avg. Cost & L1 Dist.  & Avg. Cost & L1 Dist. \\
\midrule[0.8pt]
AM Critic & 50 & 6.1153 & 144.4978& 8.8801 & 315.5329& \\
\ours{} (ours) & 50 & \textbf{6.0458} & \textbf{30.4985} & \textbf{8.726} & \textbf{49.8098} \\
\midrule[0.8pt]
AM Critic & 100 & 6.6262 & 275.9329 & 9.1065 & 569.7021 & \\
\ours{} (ours) & 100 & \textbf{6.1988} & \textbf{32.5435} & \textbf{8.6004} & \textbf{42.7087} \\
\bottomrule[1.0pt]
\end{tabular}\label{tab:sym-measure}
}


==> tables/dist_non_euclidean.tex <==

\resizebox{0.8\linewidth}{!}{
\begin{tabular}{llccccc}
\toprule[1.0pt]
 &  &  & \multicolumn{2}{c}{$N=50$} &  \multicolumn{2}{c}{$N=100$}\\
\cmidrule(lr{0.2em}){4-5}\cmidrule(lr{0.2em}){6-7}

Task & Method & Trained Size & Avg. Cost & L1 Dist.  & Avg. Cost & L1 Dist. \\
\midrule[0.8pt]
\multirow{4}{*}{ATSP} & MatNet & 50 & 
1.7894 & 10.0856 & 3.6036 & \textbf{583.4367} \\
& \ours{} (ours) & 50 & \textbf{1.7649} & \textbf{94.0299} & \textbf{3.3704} & 607.7099 \\
\cmidrule(lr{0.2em}){2-7}
& MatNet & 100 & 2.4666 & 193.0830 & 2.9467 & 428.804 \\
& \ours{} (ours) & 100 & \textbf{2.1490} & \textbf{98.5211} & \textbf{2.3023} & \textbf{194.436} \\
\midrule[0.8pt]
\multirow{4}{*}{FFSP} & MatNet & 50 & & & \\
& \ours{} (ours) & 50 &  \\
\cmidrule(lr{0.2em}){2-7}
& MatNet & 100 & \\
& \ours{} (ours) & 100 & \\
\bottomrule[1.0pt]
\end{tabular}
}


==> tables/hyperparams.tex <==
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule[1.0pt]
 & TSP & CVRP & ATSP & FFSP & MolOpt \\
\midrule
% \multicolumn{6}{c}{\textit{Common Training Parameters}} \\
% \midrule
Batch size & 100 & 100 & 100 & 100 & 64 \\
Epoch size & 10,000 & 10,000 & 10,000 & 10,000 & -\\
% Num. of epochs & 200 \\
Validation size & 10,000 & 10,000 & 10,000 & 10,000 & - \\
Learning rate scheduler & \multicolumn{4}{c}{MultiStepLR with $\gamma=0.1$} & - \\
\midrule
% \multicolumn{6}{c}{\textit{Symmetric Self-Distillation}} \\
% \midrule
Distillation scaler & 0.001 & 0.001 & 0.001 & 0.01 & 0.001 \\
Transformation width ($L$) & 1 & 1 & 1 & 1 & 1  \\
Base DRL method & AM Critic & Sym-NCO & MatNet & MatNet & REINVENT \\
% \midrule
% \multicolumn{6}{c}{\textit{Base DRL Parameters}} \\
% \midrule
% Optimizer & Adam & Adam & Adam & Adam & Adam \\
% Learning Rate & 1e-4 & 1e-4 & 4e-4 & 1e-4 \\
% Weight decay & - & - & 1e-6 & 1e-6 \\
% Num. of encode layers & 3 & 6 & 5 & 3\\ 
% Embedding dimension & 128 & 128 & 256 & 256\\
% % Tanh Clipping & 10.0 & 10.0 \\
% % Gradient Clipping & 1.0 & 1.0\\
% % Normalization & Batch & \\
% Num. augmentations & - & 8 & - & - & - \\
% Replay buffer size & - & - & - & - & 24 \\
\bottomrule[1.0pt]
\end{tabular}
}

==> tables/re_molopt_rst.tex <==
\begin{tabular}{lcccc}
\toprule
Oracle & REINVENT & \ours{} (ours) & \shortstack[c]{\ours{} w/o\\ Exp. Buffer (ours)} \\
\midrule
albuterol\_similarity 
& 0.871 $\pm$ 0.023 
& \textbf{0.914 $\pm$ 0.019} 
& 0.882 $\pm$ 0.047 \\
amlodipine\_mpo 
& 0.622 $\pm$ 0.015 
& \textbf{0.634 $\pm$ 0.021} 
& \textbf{0.634 $\pm$ 0.013 }
\\
celecoxib\_rediscovery 
& 0.661 $\pm$ 0.114 
& 0.662 $\pm$ 0.063
& \textbf{0.678 $\pm$ 0.126} \\
deco\_hop 
& 0.639 $\pm$ 0.008 
& 0.644 $\pm$ 0.005
& \textbf{0.653 $\pm$ 0.003} \\
drd2 
& 0.978 $\pm$ 0.009
& 0.978 $\pm$ 0.006
& \textbf{0.979 $\pm$ 0.005} \\
fexofenadine\_mpo 
& 0.751 $\pm$ 0.006 
& \textbf{0.770 $\pm$ 0.012} 
& 0.766 $\pm$ 0.009
\\
gsk3b 
& 0.843 $\pm$ 0.011
& 0.862 $\pm$ 0.040
& \textbf{0.876 $\pm$ 0.034} \\
isomers\_c7h8n2o2 
& 0.923 $\pm$ 0.025 
& 0.938 $\pm$ 0.021
& \textbf{0.968 $\pm$ 0.007} \\
isomers\_c9h10n2o2pf2cl 
& 0.787 $\pm$ 0.038
& 0.772 $\pm$ 0.079
& \textbf{0.887 $\pm$ 0.021} \\
jnk3 
& 0.644 $\pm$ 0.108 
& \textbf{0.666 $\pm$ 0.138}
& 0.613 $\pm$ 0.165 \\
median1 
& 0.361 $\pm$ 0.010 
& \textbf{0.369 $\pm$ 0.008} 
& 0.367 $\pm$ 0.018 
\\
median2 
& 0.268 $\pm$ 0.011 
& \textbf{0.270 $\pm$ 0.008} 
& 0.262 $\pm$ 0.013
\\
mestranol\_similarity 
& 0.670 $\pm$ 0.023
& 0.647 $\pm$ 0.022 
& \textbf{0.672 $\pm$ 0.047}
\\
osimertinib\_mpo 
& 0.832 $\pm$ 0.007 
& 0.835 $\pm$ 0.003
& \textbf{0.836 $\pm$ 0.007} \\
perindopril\_mpo 
& 0.542 $\pm$ 0.019 
& 0.543 $\pm$ 0.010
& \textbf{0.546 $\pm$ 0.017} \\
qed 
& \textbf{0.943 $\pm$ 0.000} 
& 0.942 $\pm$ 0.001 
& \textbf{0.943 $\pm$ 0.000} 
\\
ranolazine\_mpo 
& 0.778 $\pm$ 0.012 
& \textbf{0.797 $\pm$ 0.010} 
& 0.796 $\pm$ 0.011
\\
scaffold\_hop 
& 0.539 $\pm$ 0.019
& \textbf{0.579 $\pm$ 0.037} 
& 0.563 $\pm$ 0.009 
\\
sitagliptin\_mpo
& 0.423 $\pm$ 0.157
& \textbf{0.546 $\pm$ 0.047} 
& 0.516 $\pm$ 0.029
\\
thiothixene\_rediscovery 
& 0.513 $\pm$ 0.019
& \textbf{0.549 $\pm$ 0.043} 
& 0.513 $\pm$ 0.066
\\
troglitazone\_rediscovery 
& 0.364 $\pm$ 0.020
& 0.359 $\pm$ 0.016 
& \textbf{0.387 $\pm$ 0.027} 
\\
valsartan\_smarts 
& \textbf{0.000 $\pm$ 0.000} 
& \textbf{0.000 $\pm$ 0.000} 
& \textbf{0.000 $\pm$ 0.000} \\
zaleplon\_mpo 
& 0.535 $\pm$ 0.016
& 0.534 $\pm$ 0.025 
& \textbf{0.542 $\pm$ 0.016} 
\\
\midrule
Avg. & 0.630 & 0.644 & \textbf{0.647} \\
\bottomrule
\end{tabular}


==> tables/sym_distance.tex <==
\centering
\caption{L1 distances between log likelihood of symmetric action trajectories}\label{tb:sym_dist}
\begin{tabular}{ccccc}
\toprule[1.0pt]
\multicolumn{2}{c}{Scheduling} &  \multicolumn{2}{c}{Tasks}\\
\cmidrule(lr{0.2em}){1-2}\cmidrule(lr{0.2em}){3-4}
Locality& Temp. & TSP & CVRP \\
\midrule
% \\\cmidrule(lr{0.2em}){1-2}\cmidrule[0.5pt](lr{0.2em}){3-4}
  & & 18.63&63.98\\
\checkmark  & & 18.36&63.91 \\
 & \checkmark  &17.73 & 63.25\\
\checkmark  & \checkmark & \textbf{17.56}&\textbf{63.17} \\
\bottomrule[1.0pt]
\end{tabular}

